Incentives and Efficiency in Uncertain Collaborative Environments

We consider collaborative systems where users make contributions across multiple available projects and are rewarded for their contributions in individual projects according to a local sharing of the value produced. This serves as a model of online social computing systems such as online Q&A forums and of credit sharing in scientific co-authorship settings. We show that the maximum feasible produced value can be well approximated by simple local sharing rules where users are approximately rewarded in proportion to their marginal contributions and that this holds even under incomplete information about the player's abilities and effort constraints. For natural instances we show almost 95% optimality at equilibrium. When players incur a cost for their effort, we identify a threshold phenomenon: the efficiency is a constant fraction of the optimal when the cost is strictly convex and decreases with the number of players if the cost is linear.

==> introduction_-_Bak.tex <==
% !TEX root=wine13.tex

Many economic domains are ones where self-interested individuals participate in multiple joint ventures by investing time, effort, money or other personal resources, to produce some value which is then shared among the participants. Examples include traditional surplus sharing games \cite{MW96,FM99}, co-authorship settings where the wealth produced is in the form of credit in scientific projects that is implicitly split among the authors of a paper \cite{Kleinberg2011}
%, CEO labor markets where the wealth is shareholder value that is split among high-rank employers in the form of the end-of-year bonuses \cite{Nguyen2010} 
and online services contexts where users collaborate on various projects and are rewarded by means of public reputation, achievement awards, badges or webpage attention (e.g. Q\&A Forums such as Yahoo! Answers, Quora, and StackOverflow  \cite{Arpita2012a,Arpita2012b,GM12,DV09,AS09,JCP09}, open source software projects \cite{RLTRKR06,S06,KSL03,HO01,YK03}). 

Our goal is to study the global efficiency of simple and prefixed rules of sharing the value locally at each project even in the presence of incomplete information on the player's abilities and private resources constraints and even if players employ learning strategies for deciding how to play in the game. 
%The main question that we examine can be formulated as follows:
%\begin{quote}
%\emph{How should the value produced be split locally among the contributors so that the individual incentives are approximately aligned with those of the system as a whole, even in the presence of incomplete information and learning behavior?}
%\end{quote}

The design of simple, local and predetermined mechanisms is important for applications such as sharing attention in online Q\&A forums or scientific co-authorship scenarios, where cooperative game theoretic solution concepts, such as the core or bargaining, that require ad-hoc negotiations and global redistribution of value are not applicable.

Robustness to incomplete information is essential in online application settings where players hardly ever are aware of the
abilities of the players they are playing against. Instead participants have only distributional knowledge about their opponents. Additionally, public signals, such as reputation ranks, achievement boards, history of accomplishments etc. create a lot of asymmetry in the beliefs about a player's
abilities. Therefore, any efficiency guarantee should be robust to the distributional beliefs and should carry over, even if player abilities are arbitrary asymmetrically distributed. 

%We formulate a generic model of collaboration, where players have a budget of effort (e.g. time) that they are willing to spend across a set of available projects that they participate in so as to produce some value. We assume that each player has project specific abilities that determine the quality of their output at each project given some invested amount of effort. 

Our main result, is to show that as long as locally at each project, each player is awarded at least his marginal contribution to the value then every equilibrium is a $2$-approximation to the
optimal outcome and this holds even when player's abilities and budget are private information drawn from commonly known distributions and even when players use no-regret learning strategies to play the game. We portray several, simple mechanisms that satisfy this property, such as sharing proportional 
to the quality of the submission. Additionally, we give a generalization of our theorem, when players don't have hard constraints on their
resources, but rather soft constraints in the form of convex cost functions. Last we give natural classes of instances where almost
optimality is achieved at equilibrium.

%\subsection*{Our Results}

\textbf{Our Results.} We consider the following model of collaboration: the system consists of set of players and a set of projects. Each player has a budget of time that he chooses
how to distribute across his projects. If a player invests some effort at some project this results in some submission of a certain quality, which is a player and project specific increasing concave
function of the effort, that depends on the player's abilities. Each project produces some value that is a monotone submodular function of the qualities of the submissions of the different participants. This common value produced by each project is then shared among the participants of the project according to some pre-specified sharing rule, e.g. equal sharing, or sharing proportional to quality. 

\textbf{1. Marginal Contribution and Simple Sharing Rules.} We show that if each player is awarded at least his marginal contribution to the value of a project, locally, then 
every Nash equilibrium achieves at least half of the optimal social welfare. This holds at coarse correlated equilibria of the complete information game when
player's abilities and budget are common knowledge and at Bayes-Nash equilibria when these parameters are drawn independently from commonly known arbitrary distributions. Our result is based on showing that the resulting game is universally $(1,1)$-smooth game \cite{Roughgarden2012,Syrgkanis2012} and corresponds to a generalization of Vetta's \cite{Vetta2002} valid utility games
to incomplete information settings.  We give examples of simple sharing rules that satisfy the above condition, such as proportional to the marginal contribution
or based on the Shapley value or proportional to the quality.  We also show that this bound is tight for very special cases of the class of games that we study and even at pure Nash equilibria of the complete information setting. 

\textbf{2. Almost Optimality for Constant Elasticity.} We show that for the case when the value produced at each project is of the form $v(x)=w\cdot x^{\alpha}$ for $\alpha\in (0,1)$, where $x$ is the sum of the submission qualities, then the simple proportional sharing rule achieves almost 95\% of the optimal welfare at every pure Nash equilibrium of the game, which always exists.

\textbf{3. Soft Budget Constraints and a Threshold Phenomenon.} 
When the players have soft effort budget constraints in the form of some convex cost function of their total effort, we characterize the inefficiency as a function of the convexity of the cost functions, as captured by the standard measure of elasticity. We show that if the elasticity is strictly greater than $1$ (strictly convex), then the inefficiency both in terms of produced value and in terms of social welfare (including player costs) is a constant independent of the number of players, that converges to $2$ as the elasticity goes to infinity (hard budget constraint case). This stands in a stark contrast with the case when the cost functions are linear, where we show that the worst-case efficiency can decrease linearly with the number of players. 

\textbf{Applications.} In the context of social computing each project represents a specific topic on a user-generated website such as Yahoo! Answers, Quora, and StackOverflow. Each web user has
a budget of time that he spends on such a web service, which he chooses how to split among different topics/questions that arise. The quality of the response of a player
is dependent on his effort and on his abilities which are most probably private information.
The attention produced is implicitly split among the responders of the topic in a non-uniform manner, since the higher the slot that the response is placed in the feed, the higher the attention it gets. Hence, the website designer has the power to implicitly choose the attention-sharing mechanism locally at each topic, by strategically ordering the responses according to their quality and potentially randomizing, with the goal of maximizing the global attention on his web-service. 

Another interesting application of our work is in the context of sharing scientific credit in paper co-authorship scenarios. One could think of players as researchers splitting their time among different scientific projects. Given the efforts of the authors at each project there is some scientific credit produced. 
Local sharing rules in this scenario translate to scientific credit-sharing rules among the authors of a paper, which is implicitly
accomplished through the order that authors appear in the paper. Different ordering conventions in different communities correspond to different sharing mechanisms, with the alphabetical ordering corresponding to equal sharing of the credit while the contribution ordering is an instance of a sharing mechanism where a larger credit is rewarded to those who contributed more. 
%\vsdelete{Our results imply that the equal sharing rule works well only when the number of authors per paper is small. The former is reassured by the fact that communities  (e.g. theory community) that endorse the alphabetical ordering of authors in a paper, generally produce papers with a small number of co-authors.
%On the contrary, communities like physics and biology where papers can consist of as many as $30$ authors, generally order authors according to contribution.}



